Point Cloud Subsampling Parallelization for Unified Memory Platforms

The exploration of unknown environments using robots is a task that integrates different areas such as location, mapping, and planning. For mapping, there are numerous methods to represent the environments through which a robot can travel, in two and three dimensions. The probabilistic occupation grid, Octomap, and STVL can be mentioned among the most important in recent years. Nowadays, RGB-D cameras are widely used to generate a detailed representation of the environment. RGB-D camera measurements present a large volume of data, which must be reduced in order to be used in platforms with limited computing resources. This work presents an implementation of the point cloud decimation method capable of being executed on platforms with unified memory. It consists of reducing the point cloud iteratively using a subdivision of space. Results were obtained for different sizes of grids, platforms, and scenarios, both real and simulated. The results indicate that in embedded systems it is convenient to have architectures that share memory between CPU and GPU to optimize data block communication processes.

==> bib/mybib.tex <==
% Generated by IEEEtran.bst, version: 1.12 (2007/01/11)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{moravec_1985}
H.~Moravec and A.~Elfes, ``High resolution maps from wide angle sonar,'' in
  \emph{Proceedings of the IEEE international conference on robotics and
  automation ({ICRA}’85)}, 1985.

\bibitem{moravec1996}
H.~P. Moravec, ``Robot spatial perception by stereoscopic vision and 3d
  evidence grids,'' Robotics Institute, Tech. Rep., 1996.

\bibitem{dryanovski2010}
I.~{Dryanovski}, W.~{Morris}, and J.~{Xiao}, ``Multi-volume occupancy grids: An
  efficient probabilistic 3d mapping model for micro aerial vehicles,'' in
  \emph{2010 IEEE/RSJ International Conference on Intelligent Robots and
  Systems}, 2010, pp. 1553--1559.

\bibitem{hornung2013}
\BIBentryALTinterwordspacing
A.~Hornung, K.~M. Wurm, M.~Bennewitz, C.~Stachniss, and W.~Burgard,
  ``{OctoMap}: An efficient probabilistic {3D} mapping framework based on
  octrees,'' \emph{Autonomous Robots}, 2013, software available at
  \url{http://octomap.github.com}. [Online]. Available:
  \url{http://octomap.github.com}
\BIBentrySTDinterwordspacing

\bibitem{doctor1981}
L.~Doctor and J.~Torborg, ``Display techniques for octree-encoded objects,''
  \emph{IEEE Computer Graphics and Applications}, vol.~1, no.~3, pp. 29--38,
  1981.

\bibitem{museth2013vdb}
K.~Museth, ``Vdb: High-resolution sparse volumes with dynamic topology,''
  \emph{ACM transactions on graphics (TOG)}, vol.~32, no.~3, pp. 1--22, 2013.

\bibitem{museth2019}
\BIBentryALTinterwordspacing
K.~Museth, N.~Avramoussis, and D.~Bailey, ``Open{VDB},'' in \emph{ACM SIGGRAPH
  2019 Courses}, ser. SIGGRAPH '19.\hskip 1em plus 0.5em minus 0.4em\relax New
  York, NY, USA: Association for Computing Machinery, 2019. [Online].
  Available: \url{https://doi.org/10.1145/3305366.3328070}
\BIBentrySTDinterwordspacing

\bibitem{stvl2020steve}
\BIBentryALTinterwordspacing
S.~Macenski, D.~Tsai, and M.~Feinberg, ``Spatio-temporal voxel layer: A view on
  robot perception for the dynamic world,'' \emph{International Journal of
  Advanced Robotic Systems}, vol.~17, no.~2, 2020. [Online]. Available:
  \url{https://doi.org/10.1177/1729881420910530}
\BIBentrySTDinterwordspacing

\bibitem{Rusu_ICRA2011_PCL}
R.~B. Rusu and S.~Cousins, ``{3D is here: Point Cloud Library (PCL)},'' in
  \emph{{IEEE International Conference on Robotics and Automation (ICRA)}},
  Shanghai, China, May 9-13 2011.

\bibitem{bkedkowski2013general}
J.~Bedkowski, K.~Majek, and A.~Nuchter, ``General purpose computing on graphics
  processing units for robotic applications,'' \emph{Journal of Software
  Engineering for Robotics}, 2013.

\bibitem{quigley2009ROS}
M.~Quigley, ``{ROS}: an open-source robot operating system,'' in \emph{ICRA
  2009}, 2009.

\bibitem{pcl}
``Point cloud library,'' \url{https://pointclouds.org/}, accessed: 2020-09-20.

\bibitem{stvl}
``Spatio-temporal voxel layer,'' \url{https://github.com/SteveMacenski/
  spatio\_temporal\_voxel\_layer}, accessed: 2020-09-20.

\bibitem{koenig2004design}
N.~Koenig and A.~Howard, ``Design and use paradigms for gazebo, an open-source
  multi-robot simulator,'' in \emph{2004 IEEE/RSJ International Conference on
  Intelligent Robots and Systems (IROS)(IEEE Cat. No. 04CH37566)},
  vol.~3.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2004, pp. 2149--2154.

\bibitem{gazebo}
``Gazebo,'' \url{https://github.com/osrf/gazebo}, accessed: 2020-09-20.

\bibitem{foote2013}
T.~Foote, ``tf: The transform library,'' in \emph{Technologies for Practical
  Robot Applications (TePRA), 2013 IEEE International Conference on}, ser.
  Open-Source Software workshop, April 2013, pp. 1--6.

\bibitem{tbd}
E.~Marder-Eppstein, E.~Berger, T.~Foote, B.~Gerkey, and K.~Konolige, ``The
  office marathon: Robust navigation in an indoor office environment,'' in
  \emph{International Conference on Robotics and Automation}, 2010.

\bibitem{cudaSpeed}
``{cuda-samples} bandwith test,''
  \url{https://github.com/NVIDIA/cuda-samples/tree/master/Samples/bandwidthTest},
  accessed: 2020-09-10.

\bibitem{cudaTuring}
``{NVIDIA} turing architecture in-depth,''
  \url{https://developer.nvidia.com/blog/nvidia-turing-architecture-in-depth},
  accessed: 2020-09-10.

\bibitem{gvdb}
``{NVIDIA} gvdb voxels,'' \url{https://developer.nvidia.com/gvdb}, accessed:
  2020-09-10.

\end{thebibliography}

